Mixup-breakdown: a consistency training method for improving generalization of speech separation models

Deep-learning based speech separation models confront poor generalization problem that even the state-of-the-art models could abruptly fail when evaluating them in mismatch conditions. To address this problem, we propose an easy-to-implement yet effective consistency based semi-supervised learning (SSL) approach, namely Mixup-Breakdown training (MBT). It learns a teacher model to "breakdown" unlabeled inputs, and the estimated separations are interpolated to produce more useful pseudo "mixup" input-output pairs, on which the consistency regularization could apply for learning a student model. In our experiment, we evaluate MBT under various conditions with ascending degrees of mismatch, including unseen interfering speech, noise, and music, and compare MBT's generalization capability against state-of-the-art supervised learning and SSL approaches. The result indicates that MBT significantly outperforms several strong baselines with up to 13.77% relative SI-SNRi improvement. Moreover, MBT only adds negligible computational overhead to standard training schemes.

==> ICT-figure.tex <==

% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[scale=0.9,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (90.5,55) .. controls (90.5,52.24) and (92.74,50) .. (95.5,50) -- (178.5,50) .. controls (181.26,50) and (183.5,52.24) .. (183.5,55) -- (183.5,70) .. controls (183.5,72.76) and (181.26,75) .. (178.5,75) -- (95.5,75) .. controls (92.74,75) and (90.5,72.76) .. (90.5,70) -- cycle ;

%Rounded Rect [id:dp07826841282972374] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (197.5,55.6) .. controls (197.5,52.51) and (200.01,50) .. (203.1,50) -- (260.9,50) .. controls (263.99,50) and (266.5,52.51) .. (266.5,55.6) -- (266.5,72.4) .. controls (266.5,75.49) and (263.99,78) .. (260.9,78) -- (203.1,78) .. controls (200.01,78) and (197.5,75.49) .. (197.5,72.4) -- cycle ;

%Straight Lines [id:da4103657199187791] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (215.2,150) -- (277.79,187.96) ;
\draw [shift={(279.5,189)}, rotate = 211.24] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5057298337118173] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (315.5,80) -- (286.59,124.32) ;
\draw [shift={(285.5,126)}, rotate = 303.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da16279766376453575] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (235.5,78) -- (259.59,125.22) ;
\draw [shift={(260.5,127)}, rotate = 242.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Circle [id:dp3667715942513149] 
\draw   (123.25,136.5) .. controls (123.25,127.94) and (130.19,121) .. (138.75,121) .. controls (147.31,121) and (154.25,127.94) .. (154.25,136.5) .. controls (154.25,145.06) and (147.31,152) .. (138.75,152) .. controls (130.19,152) and (123.25,145.06) .. (123.25,136.5) -- cycle ;
%Straight Lines [id:da9613919403414286] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (138.5,74) -- (138.74,119) ;
\draw [shift={(138.75,121)}, rotate = 269.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7219407720159915] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (138.75,152) -- (138.52,181) ;
\draw [shift={(138.5,183)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp9576071556960143] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (283.5,56.6) .. controls (283.5,53.51) and (286.01,51) .. (289.1,51) -- (346.9,51) .. controls (349.99,51) and (352.5,53.51) .. (352.5,56.6) -- (352.5,73.4) .. controls (352.5,76.49) and (349.99,79) .. (346.9,79) -- (289.1,79) .. controls (286.01,79) and (283.5,76.49) .. (283.5,73.4) -- cycle ;

%Shape: Circle [id:dp799518940955705] 
\draw   (258.25,137.5) .. controls (258.25,128.94) and (265.19,122) .. (273.75,122) .. controls (282.31,122) and (289.25,128.94) .. (289.25,137.5) .. controls (289.25,146.06) and (282.31,153) .. (273.75,153) .. controls (265.19,153) and (258.25,146.06) .. (258.25,137.5) -- cycle ;

%Straight Lines [id:da4920668780767268] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (258.25,137.5) -- (223.5,137.5) ;
\draw [shift={(221.5,137.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp5391700666482967] 
\draw   (179.5,130.8) .. controls (179.5,128.15) and (181.65,126) .. (184.3,126) -- (215.2,126) .. controls (217.85,126) and (220,128.15) .. (220,130.8) -- (220,145.2) .. controls (220,147.85) and (217.85,150) .. (215.2,150) -- (184.3,150) .. controls (181.65,150) and (179.5,147.85) .. (179.5,145.2) -- cycle ;

%Straight Lines [id:da5817585740923171] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (178.5,136.5) -- (156.25,136.5) ;
\draw [shift={(154.25,136.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9756646858308705] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (235.5,78) -- (215.98,124.16) ;
\draw [shift={(215.2,126)}, rotate = 292.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da764947202976921] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (297.1,79) -- (221.66,129.68) ;
\draw [shift={(220,130.8)}, rotate = 326.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (137.77,61.88) node   {$(\mathbf{x}_{i} ,\ \mathbf{y}_{i}) \sim \mathcal{D}_{L}$};
% Text Node
\draw (233.6,64) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (140.5,135.75) node   {$\mathbf{f}_{\theta _{S}}$};
% Text Node
\draw (141,217) node   {$\mathcal{L}(\mathbf{y}_{i} ,\ \mathbf{f}_{\theta _{S}}(\mathbf{x}_{i}))$};
% Text Node
\draw (140,196) node  [align=left] {Goodness-of-fit};
% Text Node
\draw (331,218) node   {$\left\Vert \mathbf{f}_{\theta _{S}}\left(\text{mixup}(\mathbf{x}_{j} ,\mathbf{x}_{k})\right) -\text{mixup}(\mathbf{f}_{\theta _{T}}(\mathbf{x}_{j}) ,\mathbf{f}_{\theta _{T}}(\mathbf{x}_{k})) \ \right\Vert ^{2}_{2}$};
% Text Node
\draw (332,197) node  [align=left] {Consistency};
% Text Node
\draw (319.6,65) node   {$\mathbf{x}_{k} \sim \mathcal{D}_{U}$};
% Text Node
\draw (275.5,136.75) node   {$\mathbf{f}_{\theta _{T}}$};
% Text Node
\draw (199.75,138) node  [align=left] {mixup};


\end{tikzpicture}
}

==> MT-figure.tex <==

% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[scale=0.9,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Rounded Rect [id:dp12767908232326164] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (82.5,144) .. controls (82.5,141.24) and (84.74,139) .. (87.5,139) -- (170.5,139) .. controls (173.26,139) and (175.5,141.24) .. (175.5,144) -- (175.5,159) .. controls (175.5,161.76) and (173.26,164) .. (170.5,164) -- (87.5,164) .. controls (84.74,164) and (82.5,161.76) .. (82.5,159) -- cycle ;

%Rounded Rect [id:dp22857938512568665] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (192.5,83.6) .. controls (192.5,80.51) and (195.01,78) .. (198.1,78) -- (255.9,78) .. controls (258.99,78) and (261.5,80.51) .. (261.5,83.6) -- (261.5,100.4) .. controls (261.5,103.49) and (258.99,106) .. (255.9,106) -- (198.1,106) .. controls (195.01,106) and (192.5,103.49) .. (192.5,100.4) -- cycle ;

%Straight Lines [id:da49408415451096455] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (225.5,106) -- (224.8,134) ;
\draw [shift={(224.75,136)}, rotate = 271.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6927333200508282] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (339.5,107) -- (339.73,133) ;
\draw [shift={(339.75,135)}, rotate = 269.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da04676192261520795] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (255.9,106) -- (321.75,142.04) ;
\draw [shift={(323.5,143)}, rotate = 208.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7280993943142585] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (309.1,107) -- (241.29,141.1) ;
\draw [shift={(239.5,142)}, rotate = 333.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Circle [id:dp35584051129460037] 
\draw   (209.25,151.5) .. controls (209.25,142.94) and (216.19,136) .. (224.75,136) .. controls (233.31,136) and (240.25,142.94) .. (240.25,151.5) .. controls (240.25,160.06) and (233.31,167) .. (224.75,167) .. controls (216.19,167) and (209.25,160.06) .. (209.25,151.5) -- cycle ;
%Straight Lines [id:da8996871837680779] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (176.5,152) -- (207.25,151.53) ;
\draw [shift={(209.25,151.5)}, rotate = 539.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da939106238933185] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (224.75,167) -- (224.52,196) ;
\draw [shift={(224.5,198)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp910132505541622] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (303.5,84.6) .. controls (303.5,81.51) and (306.01,79) .. (309.1,79) -- (366.9,79) .. controls (369.99,79) and (372.5,81.51) .. (372.5,84.6) -- (372.5,101.4) .. controls (372.5,104.49) and (369.99,107) .. (366.9,107) -- (309.1,107) .. controls (306.01,107) and (303.5,104.49) .. (303.5,101.4) -- cycle ;

%Shape: Circle [id:dp02003500226539312] 
\draw   (324.25,150.5) .. controls (324.25,141.94) and (331.19,135) .. (339.75,135) .. controls (348.31,135) and (355.25,141.94) .. (355.25,150.5) .. controls (355.25,159.06) and (348.31,166) .. (339.75,166) .. controls (331.19,166) and (324.25,159.06) .. (324.25,150.5) -- cycle ;
%Straight Lines [id:da7723687890937027] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (339.75,166) -- (339.52,195) ;
\draw [shift={(339.5,197)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (129.77,150.88) node   {$(\mathbf{x}_{i} ,\ \mathbf{y}_{i}) \sim \mathcal{D}_{L}$};
% Text Node
\draw (228.6,92) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (226.5,150.75) node   {$\mathbf{f}_{\theta _{S}}$};
% Text Node
\draw (227,232) node   {$\mathcal{L}(\mathbf{y}_{i} ,\ \mathbf{f}_{\theta _{S}}(\mathbf{x}_{i}))$};
% Text Node
\draw (226,211) node  [align=left] {Goodness-of-fit};
% Text Node
\draw (340,231) node   {$\left\Vert \mathbf{f}_{\theta _{S}}(\mathbf{x}_{j}) -\mathbf{f}_{\theta _{T}}(\mathbf{x}_{k})\right\Vert^2_2$};
% Text Node
\draw (341,211) node  [align=left] {Consistency};
% Text Node
\draw (339.6,93) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (341.5,149.75) node   {$\mathbf{f}_{\theta _{T}}$};


\end{tikzpicture}
}

==> SemiSuper-ICASSP2020 final_small/ICT-figure.tex <==

% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[scale=0.9,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (90.5,55) .. controls (90.5,52.24) and (92.74,50) .. (95.5,50) -- (178.5,50) .. controls (181.26,50) and (183.5,52.24) .. (183.5,55) -- (183.5,70) .. controls (183.5,72.76) and (181.26,75) .. (178.5,75) -- (95.5,75) .. controls (92.74,75) and (90.5,72.76) .. (90.5,70) -- cycle ;

%Rounded Rect [id:dp07826841282972374] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (197.5,55.6) .. controls (197.5,52.51) and (200.01,50) .. (203.1,50) -- (260.9,50) .. controls (263.99,50) and (266.5,52.51) .. (266.5,55.6) -- (266.5,72.4) .. controls (266.5,75.49) and (263.99,78) .. (260.9,78) -- (203.1,78) .. controls (200.01,78) and (197.5,75.49) .. (197.5,72.4) -- cycle ;

%Straight Lines [id:da4103657199187791] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (215.2,150) -- (277.79,187.96) ;
\draw [shift={(279.5,189)}, rotate = 211.24] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5057298337118173] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (315.5,80) -- (286.59,124.32) ;
\draw [shift={(285.5,126)}, rotate = 303.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da16279766376453575] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (235.5,78) -- (259.59,125.22) ;
\draw [shift={(260.5,127)}, rotate = 242.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Circle [id:dp3667715942513149] 
\draw   (123.25,136.5) .. controls (123.25,127.94) and (130.19,121) .. (138.75,121) .. controls (147.31,121) and (154.25,127.94) .. (154.25,136.5) .. controls (154.25,145.06) and (147.31,152) .. (138.75,152) .. controls (130.19,152) and (123.25,145.06) .. (123.25,136.5) -- cycle ;
%Straight Lines [id:da9613919403414286] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (138.5,74) -- (138.74,119) ;
\draw [shift={(138.75,121)}, rotate = 269.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7219407720159915] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (138.75,152) -- (138.52,181) ;
\draw [shift={(138.5,183)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp9576071556960143] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (283.5,56.6) .. controls (283.5,53.51) and (286.01,51) .. (289.1,51) -- (346.9,51) .. controls (349.99,51) and (352.5,53.51) .. (352.5,56.6) -- (352.5,73.4) .. controls (352.5,76.49) and (349.99,79) .. (346.9,79) -- (289.1,79) .. controls (286.01,79) and (283.5,76.49) .. (283.5,73.4) -- cycle ;

%Shape: Circle [id:dp799518940955705] 
\draw   (258.25,137.5) .. controls (258.25,128.94) and (265.19,122) .. (273.75,122) .. controls (282.31,122) and (289.25,128.94) .. (289.25,137.5) .. controls (289.25,146.06) and (282.31,153) .. (273.75,153) .. controls (265.19,153) and (258.25,146.06) .. (258.25,137.5) -- cycle ;

%Straight Lines [id:da4920668780767268] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (258.25,137.5) -- (223.5,137.5) ;
\draw [shift={(221.5,137.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp5391700666482967] 
\draw   (179.5,130.8) .. controls (179.5,128.15) and (181.65,126) .. (184.3,126) -- (215.2,126) .. controls (217.85,126) and (220,128.15) .. (220,130.8) -- (220,145.2) .. controls (220,147.85) and (217.85,150) .. (215.2,150) -- (184.3,150) .. controls (181.65,150) and (179.5,147.85) .. (179.5,145.2) -- cycle ;

%Straight Lines [id:da5817585740923171] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (178.5,136.5) -- (156.25,136.5) ;
\draw [shift={(154.25,136.5)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9756646858308705] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (235.5,78) -- (215.98,124.16) ;
\draw [shift={(215.2,126)}, rotate = 292.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da764947202976921] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (297.1,79) -- (221.66,129.68) ;
\draw [shift={(220,130.8)}, rotate = 326.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (137.77,61.88) node   {$(\mathbf{x}_{i} ,\ \mathbf{y}_{i}) \sim \mathcal{D}_{L}$};
% Text Node
\draw (233.6,64) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (140.5,135.75) node   {$\mathbf{f}_{\theta _{S}}$};
% Text Node
\draw (141,217) node   {$\mathcal{L}(\mathbf{y}_{i} ,\ \mathbf{f}_{\theta _{S}}(\mathbf{x}_{i}))$};
% Text Node
\draw (140,196) node  [align=left] {Goodness-of-fit};
% Text Node
\draw (331,218) node   {$\left\Vert \mathbf{f}_{\theta _{S}}\left(\text{mixup}(\mathbf{x}_{j} ,\mathbf{x}_{k})\right) -\text{mixup}(\mathbf{f}_{\theta _{T}}(\mathbf{x}_{j}) ,\mathbf{f}_{\theta _{T}}(\mathbf{x}_{k})) \ \right\Vert ^{2}_{2}$};
% Text Node
\draw (332,197) node  [align=left] {Consistency};
% Text Node
\draw (319.6,65) node   {$\mathbf{x}_{k} \sim \mathcal{D}_{U}$};
% Text Node
\draw (275.5,136.75) node   {$\mathbf{f}_{\theta _{T}}$};
% Text Node
\draw (199.75,138) node  [align=left] {mixup};


\end{tikzpicture}
}

==> SemiSuper-ICASSP2020 final_small/MT-figure.tex <==

% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[scale=0.9,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Rounded Rect [id:dp12767908232326164] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (82.5,144) .. controls (82.5,141.24) and (84.74,139) .. (87.5,139) -- (170.5,139) .. controls (173.26,139) and (175.5,141.24) .. (175.5,144) -- (175.5,159) .. controls (175.5,161.76) and (173.26,164) .. (170.5,164) -- (87.5,164) .. controls (84.74,164) and (82.5,161.76) .. (82.5,159) -- cycle ;

%Rounded Rect [id:dp22857938512568665] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (192.5,83.6) .. controls (192.5,80.51) and (195.01,78) .. (198.1,78) -- (255.9,78) .. controls (258.99,78) and (261.5,80.51) .. (261.5,83.6) -- (261.5,100.4) .. controls (261.5,103.49) and (258.99,106) .. (255.9,106) -- (198.1,106) .. controls (195.01,106) and (192.5,103.49) .. (192.5,100.4) -- cycle ;

%Straight Lines [id:da49408415451096455] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (225.5,106) -- (224.8,134) ;
\draw [shift={(224.75,136)}, rotate = 271.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6927333200508282] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (339.5,107) -- (339.73,133) ;
\draw [shift={(339.75,135)}, rotate = 269.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da04676192261520795] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (255.9,106) -- (321.75,142.04) ;
\draw [shift={(323.5,143)}, rotate = 208.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7280993943142585] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (309.1,107) -- (241.29,141.1) ;
\draw [shift={(239.5,142)}, rotate = 333.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Circle [id:dp35584051129460037] 
\draw   (209.25,151.5) .. controls (209.25,142.94) and (216.19,136) .. (224.75,136) .. controls (233.31,136) and (240.25,142.94) .. (240.25,151.5) .. controls (240.25,160.06) and (233.31,167) .. (224.75,167) .. controls (216.19,167) and (209.25,160.06) .. (209.25,151.5) -- cycle ;
%Straight Lines [id:da8996871837680779] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (176.5,152) -- (207.25,151.53) ;
\draw [shift={(209.25,151.5)}, rotate = 539.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da939106238933185] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (224.75,167) -- (224.52,196) ;
\draw [shift={(224.5,198)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp910132505541622] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]  (303.5,84.6) .. controls (303.5,81.51) and (306.01,79) .. (309.1,79) -- (366.9,79) .. controls (369.99,79) and (372.5,81.51) .. (372.5,84.6) -- (372.5,101.4) .. controls (372.5,104.49) and (369.99,107) .. (366.9,107) -- (309.1,107) .. controls (306.01,107) and (303.5,104.49) .. (303.5,101.4) -- cycle ;

%Shape: Circle [id:dp02003500226539312] 
\draw   (324.25,150.5) .. controls (324.25,141.94) and (331.19,135) .. (339.75,135) .. controls (348.31,135) and (355.25,141.94) .. (355.25,150.5) .. controls (355.25,159.06) and (348.31,166) .. (339.75,166) .. controls (331.19,166) and (324.25,159.06) .. (324.25,150.5) -- cycle ;
%Straight Lines [id:da7723687890937027] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (339.75,166) -- (339.52,195) ;
\draw [shift={(339.5,197)}, rotate = 270.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (129.77,150.88) node   {$(\mathbf{x}_{i} ,\ \mathbf{y}_{i}) \sim \mathcal{D}_{L}$};
% Text Node
\draw (228.6,92) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (226.5,150.75) node   {$\mathbf{f}_{\theta _{S}}$};
% Text Node
\draw (227,232) node   {$\mathcal{L}(\mathbf{y}_{i} ,\ \mathbf{f}_{\theta _{S}}(\mathbf{x}_{i}))$};
% Text Node
\draw (226,211) node  [align=left] {Goodness-of-fit};
% Text Node
\draw (340,231) node   {$\left\Vert \mathbf{f}_{\theta _{S}}(\mathbf{x}_{j}) -\mathbf{f}_{\theta _{T}}(\mathbf{x}_{k})\right\Vert^2_2$};
% Text Node
\draw (341,211) node  [align=left] {Consistency};
% Text Node
\draw (339.6,93) node   {$\mathbf{x}_{j} \sim \mathcal{D}_{U}$};
% Text Node
\draw (341.5,149.75) node   {$\mathbf{f}_{\theta _{T}}$};


\end{tikzpicture}
}
